Search for the Blazhko effect in field RR Lyrae stars using LINEAR and ZTF light curves

We analyzed the incidence and properties of RR Lyrae stars that show evidence for amplitude and phase modulation (the so-called Blazhko Effect) in a sample of $\sim$3,000 stars with LINEAR and ZTF light curve data collected during the periods of 2002-2008 and 2018-2023, respectively. A preliminary subsample of about $\sim$500 stars was algorithmically pre-selected using various data quality and light curve statistics, and then 228 stars were confirmed visually as displaying the Blazhko effect. This sample increases the number of field RR Lyrae stars displaying the Blazhko effect by more than 50\% and places a lower limit of (11.4$\pm$0.8)\% for their incidence rate. We find that ab type RR Lyrae that show the Blazhko effect have about 5\% (0.030 day) shorter periods than starting sample, a 7.1$\sigma$ statistically significant difference. We find no significant differences in their light curve amplitudes and apparent magnitude (essentially, signal-to-noise ratio) distributions. No period or other differences are found for c type RR Lyrae. We find convincing examples of stars where the Blazhko effect can appear and disappear on time scales of several years. With time-resolved photometry expected from LSST, a similar analysis will be performed for even larger samples of field RR Lyrae stars in the southern sky and we anticipate a higher fraction of discovered Blazhko stars due to better sampling and superior photometric quality.

==> be_full.tex <==
\begin{center}
%\footnotesize
\scriptsize
\begin{tabular}{rccrrccrrrrrrrrrrlrr}
\toprule
 LID &  P$_L$ &   P$_Z$ &  N$_L$ &  N$_Z$&  $\chi^2_{L,r}$ &  $\chi^2_{Z,r}$ &  $\chi^2_L$ &  $\chi^2_Z$ & $A_L$ &  $A_Z$ &  $\delta$A &  Bp$_L$ &  Bp$_Z$ &  Bp$_L$ &  Bp$_Z$ &  t &  f &  B\_s & B\_f \\
\midrule
    158779 & 0.609207 & 0.609189 &  293 &  616 &      1.6 &      3.9 &     3.7 &    34.2 &   0.47 &   0.68 &       0.21 &  1.6443 &  1.6444 &  352.7337 &  350.2627 &       1 &             - &        7 &         1 \\
    263541 & 0.558218 & 0.558221 &  270 &  503 &      2.9 &      6.6 &    15.8 &   110.4 &   0.64 &   0.82 &       0.18 &  1.8621 &  1.8025 &   14.1513 &   89.9685 &       1 &             - &        7 &         1 \\
    393084 & 0.530027 & 0.530033 &  493 &  372 &      1.1 &      3.2 &     1.6 &    19.2 &   0.96 &   1.31 &       0.35 &  1.9447 &  1.8896 &   17.2369 &  347.2222 &       1 &             - &        6 &         1 \\
    810169 & 0.465185 & 0.465212 &  289 &  743 &      2.1 &      2.8 &     6.0 &    15.1 &   0.77 &   0.75 &       0.02 &  2.2232 &  2.2230 &   13.6017 &   13.6082 &       1 &             - &        5 &         1 \\
    924301 & 0.507503 & 0.507440 &  418 &  189 &      1.9 &      9.3 &    13.8 &   162.9 &   0.87 &   0.79 &       0.08 &  2.0043 &  1.9763 &   29.5072 &  178.4121 &       1 &             - &        8 &         1 \\
    970326 & 0.592233 & 0.592231 &  275 &  552 &      1.1 &      2.1 &     1.9 &     7.7 &   0.51 &   0.75 &       0.24 &  1.7563 &  1.6992 &   14.7656 &   93.2836 &       1 &             - &        5 &         1 \\
    999528 & 0.658401 & 0.658407 &  564 &  213 &      1.2 &      2.7 &     1.8 &    21.7 &   0.57 &   0.92 &       0.35 &  1.5527 &  1.5510 &   29.5247 &   31.0366 &       1 &             - &        5 &         1 \\
   1005497 & 0.653607 & 0.653605 &  607 &  192 &      1.1 &      2.1 &     2.1 &    12.4 &   0.60 &   0.83 &       0.23 &  1.5639 &  1.5481 &   29.4638 &   55.1116 &       1 &             - &        5 &         1 \\
   1092244 & 0.649496 & 0.649558 &  590 &  326 &      1.2 &      3.6 &     2.3 &    32.1 &   0.72 &   0.58 &       0.14 &  1.5735 &  1.5640 &   29.5421 &   40.8330 &       1 &             - &        7 &         1 \\
   1240665 & 0.632528 & 0.632522 &  468 &  311 &      3.0 &      1.1 &    25.2 &     1.6 &   0.33 &   0.33 &       0.00 &  1.6149 &  1.5865 &   29.4942 &  182.3154 &       1 &             Z &        0 &         2 \\
   1244554 & 0.536875 & 0.536962 &  469 &  312 &      1.8 &      2.3 &     9.5 &    14.8 &   0.71 &   0.97 &       0.26 &  1.8966 &  1.9325 &   29.4638 &   14.2481 &       1 &             - &        7 &         1 \\
   1271119 & 0.565270 & 0.565257 &  280 &  521 &      1.0 &      4.0 &     2.9 &    45.5 &   0.69 &   0.90 &       0.21 &  1.8366 &  1.7739 &   14.8060 &  208.3333 &       1 &             - &        6 &         1 \\
   1332201 & 0.580711 & 0.580731 &  260 &  208 &      1.6 &      4.2 &     9.2 &    50.1 &   0.59 &   0.83 &       0.24 &  1.7559 &  1.7918 &   29.4942 &   14.3225 &       1 &             - &        7 &         1 \\
   1390653 & 0.521867 & 0.521871 &  524 &  310 &      1.3 &      4.1 &     4.2 &    44.9 &   1.10 &   1.28 &       0.18 &  1.9502 &  2.0026 &   29.4291 &   11.5768 &       1 &             - &        6 &         1 \\
   1448299 & 0.606912 & 0.606940 &  435 &  267 &      2.7 &      5.4 &    32.5 &    35.6 &   0.77 &   0.70 &       0.07 &  1.6816 &  1.6531 &   29.4551 &  180.9955 &       1 &             - &        8 &         1 \\
   1539000 & 0.500288 & 0.500279 &  410 &  468 &      1.5 &      3.6 &     6.1 &    66.3 &   0.89 &   1.13 &       0.24 &  2.0021 &  2.0017 &  303.9514 &  355.8719 &       1 &             - &        6 &         1 \\
   1593736 & 0.592628 & 0.592650 &  264 &  532 &      1.2 &      5.7 &     2.1 &    35.9 &   0.37 &   0.36 &       0.01 &  1.7584 &  1.6910 &   14.0795 &  272.4796 &       1 &             - &        6 &         1 \\
   1748058 & 0.310237 & 0.310176 &  463 &  272 &      1.4 &      5.7 &     2.2 &    30.7 &   0.38 &   0.23 &       0.15 &  3.2572 &  3.2297 &   29.5203 &  173.3102 &       2 &             - &        7 &         1 \\
   1790596 & 0.534498 & 0.534506 &  509 &  327 &      3.1 &      3.3 &    19.3 &    15.6 &   0.79 &   0.70 &       0.09 &  1.9046 &  1.8764 &   29.6868 &  182.1494 &       1 &             - &        6 &         1 \\
   1882354 & 0.695061 & 0.695029 &  313 &  411 &      1.5 &      2.8 &     3.0 &    13.2 &   0.63 &   0.70 &       0.07 &  1.4909 &  1.4419 &   19.1516 &  326.2643 &       1 &             - &        6 &         1 \\
   1936459 & 0.649248 & 0.649240 &  431 &  268 &      0.7 &      1.1 &     0.6 &     1.7 &   0.45 &   0.43 &       0.02 &  1.5741 &  1.5458 &   29.5203 &  181.8182 &       1 &             Z &        0 &         2 \\
   2041979 & 0.653694 & 0.653639 &  276 & 1378 &      1.2 &      5.3 &     1.5 &    57.5 &   0.63 &   0.64 &       0.01 &  1.5944 &  1.5816 &   15.4607 &   19.3442 &       1 &             - &        7 &         1 \\
   2050107 & 0.686454 & 0.686466 &  190 & 1388 &      3.9 &      3.3 &    16.4 &    22.3 &   0.78 &   0.64 &       0.14 &  1.4906 &  1.4633 &   29.5159 &  151.2859 &       1 &             - &        6 &         1 \\
   2122319 & 0.359422 & 0.359424 &  519 &  199 &      2.1 &      6.1 &     7.2 &    36.6 &   0.38 &   0.55 &       0.17 &  2.8161 &  2.8926 &   29.5421 &    9.0645 &       2 &             - &        7 &         1 \\
   2229607 & 0.575179 & 0.575211 &  290 &  731 &      1.2 &      4.4 &     2.7 &    38.3 &   0.55 &   0.81 &       0.26 &  1.8093 &  1.7433 &   14.1383 &  207.2539 &       1 &             - &        8 &         1 \\
   2243683 & 0.579777 & 0.579803 &  531 &  262 &      3.1 &      4.3 &    22.0 &    36.0 &   0.52 &   0.56 &       0.04 &  1.7588 &  1.7303 &   29.4204 &  180.0180 &       1 &             - &        6 &         1 \\
   2264042 & 0.655373 & 0.655391 &  391 &  299 &      1.6 &      4.0 &     6.5 &    57.4 &   0.74 &   0.76 &       0.02 &  1.5597 &  1.5313 &   29.5465 &  182.4818 &       1 &             - &        5 &         1 \\
   2280940 & 0.562372 & 0.562374 &  310 &  735 &      1.1 &      3.2 &     1.4 &    17.5 &   0.84 &   1.01 &       0.17 &  1.8461 &  1.7847 &   14.7286 &  153.2567 &       1 &             - &        6 &         1 \\
   2333087 & 0.551462 & 0.551424 &  560 &  202 &      3.5 &      8.0 &    29.8 &    90.2 &   0.72 &   0.88 &       0.16 &  1.8473 &  1.8304 &   29.5072 &   59.0842 &       1 &             - &        9 &         1 \\
   2334384 & 0.555341 & 0.555333 &  443 &  204 &      2.0 &      6.5 &    10.5 &    84.7 &   0.63 &   0.88 &       0.25 &  1.8346 &  1.8353 &   29.5377 &   28.9394 &       1 &             - &        7 &         1 \\
   2397296 & 0.488814 & 0.488836 &  522 &  196 &      1.2 &      6.6 &     3.2 &    78.9 &   0.65 &   1.01 &       0.36 &  2.0796 &  2.0672 &   29.5421 &   46.5224 &       1 &             - &        9 &         1 \\
   2414841 & 0.559611 & 0.559592 &  522 &  305 &      1.7 &      5.7 &     5.6 &    62.8 &   0.69 &   1.09 &       0.40 &  1.8208 &  1.7920 &   29.5421 &  201.2072 &       1 &             - &        8 &         1 \\
   2612592 & 0.571562 & 0.571543 &  270 & 1391 &      1.3 &      2.8 &     2.4 &    24.8 &   0.76 &   0.70 &       0.06 &  1.8173 &  1.7544 &   14.7787 &  208.5506 &       1 &             - &        5 &         1 \\
   2683009 & 0.606278 & 0.606210 &  180 &  892 &      6.6 &      7.4 &    63.6 &    88.8 &   0.82 &   0.52 &       0.30 &  1.6833 &  1.6603 &   29.4942 &   93.7207 &       1 &             - &        9 &         1 \\
   2851826 & 0.521838 & 0.521842 &  257 &  653 &      1.0 &      2.5 &     1.6 &    18.1 &   0.95 &   1.21 &       0.26 &  1.9595 &  1.9595 &   23.1642 &   23.1374 &       1 &             - &        5 &         1 \\
   2889542 & 0.570913 & 0.570911 &  457 &  170 &      1.3 &      2.5 &     2.7 &     9.2 &   0.96 &   1.35 &       0.39 &  1.7855 &  1.8062 &   29.4855 &   18.3268 &       1 &             - &        5 &         1 \\
   2892940 & 0.539855 & 0.539896 &  462 &  169 &      1.3 &      4.2 &     3.7 &    49.1 &   0.90 &   1.21 &       0.31 &  1.8862 &  1.9288 &   29.5290 &   13.0514 &       1 &             - &        8 &         1 \\
   2936953 & 0.328746 & 0.328733 &  271 &  187 &      2.7 &      1.3 &    13.0 &     2.5 &   0.35 &   0.29 &       0.06 &  3.1123 &  3.0448 &   14.1995 &  356.5062 &       2 &             - &        5 &         1 \\
   3140139 & 0.304590 & 0.304585 &  255 &  343 &      2.5 &      5.6 &     7.7 &    25.1 &   0.40 &   0.60 &       0.20 &  3.3529 &  3.4219 &   14.3338 &    7.2056 &       2 &             - &        7 &         1 \\
   3183285 & 0.349653 & 0.349664 &  485 &  588 &      1.2 &      2.8 &     4.1 &    15.7 &   0.48 &   0.58 &       0.10 &  2.8939 &  2.8654 &   29.4768 &  181.8182 &       2 &             - &        5 &         1 \\
   3196582 & 0.268017 & 0.268018 &  479 &  172 &      2.5 &      3.4 &     8.6 &    10.1 &   0.35 &   0.51 &       0.16 &  3.7650 &  3.8361 &   29.5203 &    9.5256 &       2 &             - &        6 &         1 \\
   3196780 & 0.504148 & 0.504199 &  475 &  286 &      2.2 &      3.2 &     9.3 &    21.5 &   0.81 &   0.85 &       0.04 &  2.0029 &  1.9889 &   51.7331 &  181.6530 &       1 &             - &        6 &         1 \\
   3219035 & 0.326746 & 0.326509 &  376 &  168 &      3.9 &      2.6 &    23.9 &    11.5 &   0.32 &   0.23 &       0.09 &  3.1287 &  3.0661 &   14.6692 &  294.1176 &       2 &             - &        7 &         1 \\
   3463199 & 0.334718 & 0.334710 &  297 &  579 &      0.7 &      2.3 &     0.6 &    11.3 &   0.51 &   0.67 &       0.16 &  3.0584 &  2.9952 &   14.1153 &  133.2445 &       2 &             - &        5 &         1 \\
   3491287 & 0.490986 & 0.490995 &  483 &  504 &      1.4 &      3.8 &     4.1 &    37.9 &   0.94 &   0.80 &       0.14 &  2.0537 &  2.0537 &   58.8408 &   58.8755 &       1 &             - &        5 &         1 \\
   3589854 & 0.612893 & 0.612953 &  468 &  545 &      3.9 &      5.8 &    29.1 &    45.0 &   0.49 &   0.50 &       0.01 &  1.6656 &  1.6369 &   29.4031 &  184.6722 &       1 &             - &        7 &         1 \\
   3591037 & 0.558643 & 0.558609 &  449 &  544 &      1.3 &      3.5 &     5.4 &    30.1 &   0.76 &   0.65 &       0.11 &  1.7929 &  1.7956 &  352.1127 &  182.3154 &       1 &             - &        7 &         1 \\
   3632428 & 0.710123 & 0.710081 &  216 & 1400 &      0.9 &      1.5 &     1.1 &     2.9 &   0.39 &   0.54 &       0.15 &  1.4121 &  1.4148 &  254.4529 &  153.9646 &       1 &             L &        0 &         2 \\
   3941776 & 0.532222 & 0.532209 &  271 &  549 &      2.8 &      6.0 &    18.8 &    89.0 &   0.77 &   0.61 &       0.16 &  1.9253 &  1.8844 &   21.5564 &  184.1621 &       1 &             - &        7 &         1 \\
   3960704 & 0.645879 & 0.645834 &  297 &  671 &      1.6 &      2.6 &     4.6 &    20.6 &   0.72 &   0.70 &       0.02 &  1.5850 &  1.5539 &   27.2442 &  182.9826 &       1 &             - &        5 &         1 \\
   4101289 & 0.379225 & 0.379250 &  256 &  657 &      1.2 &      2.7 &     2.0 &     9.0 &   0.39 &   0.37 &       0.02 &  2.7048 &  2.6416 &   14.7308 &  209.2050 &       2 &             - &        5 &         1 \\
   4234952 & 0.566338 & 0.566348 &  461 &  179 &      0.9 &      3.6 &     1.5 &    27.3 &   0.59 &   0.77 &       0.18 &  1.7995 &  1.7712 &   29.5727 &  180.1802 &       1 &             - &        6 &         1 \\
   4282396 & 0.392234 & 0.392238 &  311 &  885 &      2.4 &      5.9 &    11.6 &    47.1 &   0.51 &   0.54 &       0.03 &  2.5833 &  2.5550 &   29.5465 &  181.1594 &       2 &             - &        5 &         1 \\
   4320492 & 0.361005 & 0.360942 &  480 &  290 &      3.7 &      1.8 &    15.1 &    11.2 &   0.26 &   0.29 &       0.03 &  2.8039 &  2.7761 &   29.5116 &  180.9955 &       2 &             - &        6 &         1 \\
   4327168 & 0.330944 & 0.330937 &  482 &  182 &      1.1 &      2.8 &     1.4 &    11.3 &   0.39 &   0.56 &       0.17 &  3.0555 &  3.0299 &   29.5116 &  121.8769 &       2 &             - &        5 &         1 \\
   4512465 & 0.533053 & 0.533051 &  233 & 1039 &      1.1 &      3.4 &     4.3 &    47.6 &   0.83 &   1.13 &       0.30 &  1.9255 &  1.9394 &   20.1816 &   15.7791 &       1 &             - &        6 &         1 \\
   4551971 & 0.532348 & 0.532366 &  291 &  582 &      1.1 &      3.7 &     1.9 &    53.4 &   0.98 &   1.24 &       0.26 &  1.9406 &  1.9406 &   16.1005 &   16.0862 &       1 &             - &        7 &         1 \\
   4804945 & 0.556172 & 0.556217 &  279 &  889 &      2.5 &      7.8 &    12.5 &   100.5 &   0.58 &   0.56 &       0.02 &  1.8683 &  1.8017 &   14.2268 &  258.3979 &       1 &             - &        7 &         1 \\
   4912051 & 0.571577 & 0.571435 &  638 &  311 &      2.1 &      8.2 &     9.4 &   133.5 &   0.63 &   0.70 &       0.07 &  1.7835 &  1.7528 &   29.4855 &  356.5062 &       1 &             - &        8 &         1 \\
   5168861 & 0.597417 & 0.597442 &  198 &  691 &      1.7 &      3.1 &     5.0 &    21.9 &   0.59 &   0.58 &       0.01 &  1.7168 &  1.6793 &   23.3127 &  180.3427 &       1 &             - &        5 &         1 \\
   5308437 & 0.462680 & 0.462679 &  365 &  634 &      3.7 &      2.5 &    88.0 &    16.6 &   0.92 &   1.08 &       0.16 &  2.2406 &  2.2407 &   12.6119 &   12.6056 &       1 &             - &        6 &         1 \\
   5421989 & 0.534510 & 0.534527 &  288 & 2670 &      0.8 &      2.5 &     0.8 &    13.5 &   0.76 &   0.85 &       0.09 &  1.9414 &  1.9368 &   14.1884 &   15.1561 &       1 &             - &        5 &         1 \\
   5424357 & 0.517283 & 0.517280 &  240 & 1096 &      1.0 &      2.8 &     1.3 &    22.9 &   0.85 &   1.15 &       0.30 &  2.0037 &  1.9680 &   14.1814 &   28.7315 &       1 &             - &        5 &         1 \\
   5530643 & 0.490349 & 0.490334 &  545 &  658 &      0.9 &      2.2 &     1.8 &    14.7 &   1.24 &   0.98 &       0.26 &  2.0733 &  2.0424 &   29.4768 &  339.5586 &       1 &             - &        6 &         1 \\
   5692103 & 0.583147 & 0.583149 &  375 &  884 &      1.2 &      3.4 &     3.2 &    23.7 &   1.04 &   0.83 &       0.21 &  1.7176 &  1.7232 &  357.7818 &  119.3317 &       1 &             - &        6 &         1 \\
   5844704 & 0.530367 & 0.530401 &  197 & 1506 &      1.5 &      3.1 &     1.9 &    19.1 &   0.97 &   0.56 &       0.41 &  1.9387 &  1.9440 &   18.7811 &   17.0459 &       1 &             - &        8 &         1 \\
   5931160 & 0.664700 & 0.664708 &  587 &  658 &      0.8 &      1.1 &     0.9 &     1.3 &   0.35 &   0.33 &       0.02 &  1.5383 &  1.5078 &   29.5421 &  293.6858 &       1 &             Z &        0 &         2 \\
   5977769 & 0.555959 & 0.555952 &  359 &  795 &      1.1 &      3.2 &     1.7 &    22.1 &   0.82 &   0.94 &       0.12 &  1.8325 &  1.8016 &   29.5814 &  349.0401 &       1 &             - &        5 &         1 \\
   6022777 & 0.495745 & 0.495724 &  572 &  328 &      1.6 &      4.2 &     8.2 &    44.3 &   1.01 &   1.34 &       0.33 &  2.0244 &  2.0245 &  138.6963 &  138.6001 &       1 &             - &        7 &         1 \\
   6248770 & 0.486017 & 0.486023 &  516 &  228 &      2.0 &      3.7 &    11.0 &    80.4 &   0.88 &   1.22 &       0.34 &  2.0941 &  2.0849 &   27.3560 &   36.5631 &       1 &             - &        6 &         1 \\
   6651516 & 0.308488 & 0.308496 &  426 &  448 &      1.3 &      5.8 &     2.1 &    60.9 &   0.36 &   0.48 &       0.12 &  3.2755 &  3.3595 &   29.4724 &    8.4767 &       2 &             - &        7 &         1 \\
   6819457 & 0.436282 & 0.436265 &  325 & 1358 &      3.6 &      9.6 &    32.5 &   121.2 &   0.95 &   0.79 &       0.16 &  2.2950 &  2.3005 &  346.0208 &  120.0480 &       2 &             - &        8 &         1 \\
   6844511 & 0.591013 & 0.591001 &  241 &  571 &      1.4 &      4.6 &     5.5 &    38.6 &   0.96 &   0.89 &       0.07 &  1.7260 &  1.6950 &   29.4334 &  337.2681 &       1 &             - &        5 &         1 \\
   6967017 & 0.529691 & 0.529677 &  323 &  231 &      2.3 &      6.9 &    13.3 &    70.6 &   0.63 &   0.96 &       0.33 &  1.9218 &  1.9467 &   29.4724 &   17.0111 &       1 &             - &        8 &         1 \\
   7048826 & 0.317781 & 0.317790 &  535 &  597 &      1.4 &      5.9 &     4.0 &    55.3 &   0.50 &   0.46 &       0.04 &  3.1807 &  3.1497 &   29.4942 &  338.4095 &       2 &             - &        6 &         1 \\
   7119535 & 0.576808 & 0.576796 &  623 &  276 &      0.9 &      3.5 &     1.8 &    30.2 &   0.50 &   0.84 &       0.34 &  1.7676 &  1.7365 &   29.4855 &  353.3569 &       1 &             - &        6 &         1 \\
   7337289 & 0.404115 & 0.404114 &  552 &  248 &      1.7 &      3.9 &     4.4 &    25.4 &   0.37 &   0.51 &       0.14 &  2.5084 &  2.5550 &   29.5508 &   12.4285 &       2 &             - &        5 &         1 \\
   7344401 & 0.330201 & 0.330226 &  397 & 1164 &      1.8 &      2.7 &     5.9 &    22.0 &   0.36 &   0.48 &       0.12 &  3.1300 &  3.0393 &    9.8449 &   89.9281 &       2 &             - &        6 &         1 \\
   7510192 & 0.647056 & 0.647048 &  561 &  620 &      1.4 &      3.9 &     5.9 &    27.3 &   0.53 &   0.60 &       0.07 &  1.5794 &  1.5538 &   29.4985 &  120.5546 &       1 &             - &        5 &         1 \\
   7545954 & 0.555952 & 0.555959 &  228 &  912 &      3.7 &      3.8 &    29.7 &    20.8 &   0.81 &   0.77 &       0.04 &  1.8087 &  1.8021 &  100.0500 &  296.2963 &       1 &             L &        0 &         2 \\
   7553128 & 0.622806 & 0.622799 &  213 &  820 &      1.0 &      2.8 &     1.0 &     8.8 &   0.38 &   0.57 &       0.19 &  1.6755 &  1.6743 &   14.3133 &   14.5624 &       1 &             - &        5 &         1 \\
   7657340 & 0.495480 & 0.495493 &  482 &  511 &      2.3 &      4.0 &    11.8 &    31.0 &   0.79 &   0.73 &       0.06 &  2.0274 &  2.0259 &  109.1703 &  129.9545 &       1 &             - &        6 &         1 \\
   7716220 & 0.563336 & 0.563335 &  459 &  282 &      1.7 &      3.5 &     6.1 &    26.0 &   0.66 &   0.54 &       0.12 &  1.7779 &  1.7806 &  357.1429 &  182.3154 &       1 &             - &        5 &         1 \\
   7723614 & 0.560912 & 0.560908 &  533 &  388 &      1.1 &      2.4 &     2.8 &    16.2 &   0.74 &   1.01 &       0.27 &  1.8167 &  1.8561 &   29.4942 &   13.6454 &       1 &             - &        5 &         1 \\
   7811366 & 0.489523 & 0.489521 &  253 & 1119 &      2.0 &      4.7 &    11.4 &    62.0 &   0.81 &   1.08 &       0.27 &  2.1151 &  2.0629 &   13.8293 &   49.8504 &       1 &             - &        6 &         1 \\
   7836810 & 0.547266 & 0.547317 &  362 &  324 &      3.5 &      3.7 &    11.9 &    25.8 &   0.46 &   0.44 &       0.02 &  1.8611 &  1.8326 &   29.5247 &  182.4818 &       1 &             - &        7 &         1 \\
   7846640 & 0.551495 & 0.551518 &  447 &  178 &      1.5 &      9.2 &     5.3 &   109.1 &   0.76 &   0.81 &       0.05 &  1.8942 &  1.8236 &   12.3472 &   96.0615 &       1 &             - &        6 &         1 \\
   7997579 & 0.486693 & 0.486689 &  465 &  284 &      1.3 &      5.1 &     2.6 &    37.2 &   0.77 &   0.77 &       0.00 &  2.0886 &  2.0807 &   29.4551 &   38.4837 &       1 &             - &        5 &         1 \\
   8036191 & 0.363860 & 0.363893 &  438 &  175 &      2.2 &      1.6 &     7.8 &    10.9 &   0.40 &   0.60 &       0.20 &  2.7822 &  2.8768 &   29.5116 &    7.7688 &       2 &             - &        7 &         1 \\
   8214374 & 0.487303 & 0.487291 &  264 &  901 &      1.2 &      3.5 &     3.1 &    33.8 &   0.79 &   0.70 &       0.09 &  2.1014 &  2.0769 &   20.2963 &   40.4040 &       1 &             - &        5 &         1 \\
   8222011 & 0.350920 & 0.350914 &  264 &  729 &      2.0 &      4.8 &     5.2 &    25.2 &   0.46 &   0.35 &       0.11 &  2.8923 &  2.8532 &   23.4247 &  284.4950 &       2 &             - &        5 &         1 \\
   8311517 & 0.523354 & 0.523359 &  331 &  257 &      1.8 &      3.6 &    11.4 &    48.6 &   0.74 &   0.99 &       0.25 &  1.9567 &  1.9567 &   21.7533 &   21.7439 &       1 &             - &        6 &         1 \\
   8342007 & 0.469585 & 0.469589 &  491 &  208 &      2.0 &      3.4 &     9.2 &    26.8 &   0.93 &   1.28 &       0.35 &  2.1634 &  2.1930 &   29.5770 &   15.7629 &       1 &             - &        6 &         1 \\
   8343291 & 0.569785 & 0.569791 &  474 &  288 &      3.3 &      5.1 &    31.4 &    63.3 &   0.70 &   0.68 &       0.02 &  1.7888 &  1.7605 &   29.6121 &  181.4882 &       1 &             - &        5 &         1 \\
   8574195 & 0.576044 & 0.576038 &  188 & 1550 &      1.7 &      4.3 &     8.9 &    40.9 &   0.64 &   0.52 &       0.12 &  1.7696 &  1.7414 &   29.7089 &  185.0139 &       1 &             - &        5 &         1 \\
   8669917 & 0.554217 & 0.554210 &  228 &  502 &      2.1 &      5.1 &    11.6 &    34.0 &   0.79 &   0.97 &       0.18 &  1.8750 &  1.8194 &   14.1513 &   66.3790 &       1 &             - &        7 &         1 \\
   8738578 & 0.631217 & 0.631243 &  277 &  641 &      0.7 &      2.9 &     0.7 &     8.9 &   0.32 &   0.44 &       0.12 &  1.6228 &  1.5891 &   25.9370 &  204.7083 &       1 &             - &        5 &         1 \\
   8745173 & 0.489914 & 0.490045 &  296 &  201 &      1.9 &      4.8 &     6.0 &    41.5 &   0.71 &   1.11 &       0.40 &  2.1152 &  2.0786 &   13.5071 &   26.3089 &       2 &             - &        8 &         1 \\
   8750363 & 0.561315 & 0.561305 &  295 &  294 &      1.4 &      3.2 &     4.2 &    28.8 &   0.89 &   0.67 &       0.22 &  1.8553 &  1.7870 &   13.5593 &  183.3181 &       1 &             - &        6 &         1 \\
   8786633 & 0.677380 & 0.677441 &  202 &  605 &      2.2 &      5.5 &    11.8 &    54.4 &   0.49 &   0.68 &       0.19 &  1.4939 &  1.4811 &   56.6733 &  202.2245 &       1 &             - &        9 &         1 \\
   8797911 & 0.539254 & 0.539393 &  244 &  843 &      2.4 &      2.6 &    13.8 &    18.0 &   0.50 &   0.82 &       0.32 &  1.8572 &  1.9283 &  356.5062 &   13.4463 &       1 &             - &        7 &         1 \\
   8867725 & 0.505451 & 0.505352 &  218 &  805 &      1.1 &      6.5 &     2.4 &    96.3 &   0.90 &   0.59 &       0.31 &  2.0461 &  1.9907 &   14.7710 &   84.0689 &       1 &             - &        9 &         1 \\
   8955278 & 0.547521 & 0.547514 &  200 &  378 &      1.3 &      1.9 &     3.8 &     6.3 &   0.87 &   0.86 &       0.01 &  1.8412 &  1.8402 &   67.5904 &   72.7273 &       1 &             L &        0 &         2 \\
   9041967 & 0.587104 & 0.587101 &  224 &  503 &      1.4 &      3.7 &     3.8 &    38.0 &   0.54 &   0.78 &       0.24 &  1.7215 &  1.7082 &   54.7495 &  203.6660 &       1 &             - &        6 &         1 \\
   9063194 & 0.575781 & 0.575760 &  467 &  283 &      2.4 &      3.1 &    16.1 &    24.2 &   0.83 &   0.65 &       0.18 &  1.7707 &  1.7424 &   29.4898 &  179.3722 &       1 &             - &        7 &         1 \\
   9357148 & 0.539892 & 0.539866 &  248 &  319 &      1.6 &      5.1 &     3.9 &    76.3 &   0.69 &   0.52 &       0.17 &  1.9275 &  1.9275 &   13.2846 &   13.2926 &       1 &             - &        9 &         1 \\
   9399448 & 0.527622 & 0.527621 &  226 &  496 &      1.3 &      2.3 &     3.1 &    10.9 &   0.75 &   0.55 &       0.20 &  1.9490 &  1.9490 &   18.6202 &   18.6220 &       1 &             - &        5 &         1 \\
   9852554 & 0.651339 & 0.651367 &  339 &  217 &      1.0 &      4.5 &     1.1 &    46.6 &   0.67 &   0.75 &       0.08 &  1.5570 &  1.6001 &   46.0617 &   15.4048 &       1 &             - &        6 &         1 \\
   9918809 & 0.479460 & 0.479509 &  265 &  601 &      1.9 &     11.6 &     7.8 &   161.8 &   0.60 &   0.58 &       0.02 &  2.1556 &  2.0990 &   14.3113 &   73.7735 &       1 &             - &        7 &         1 \\
   9968431 & 0.302266 & 0.302211 &  273 &  323 &      1.7 &      2.2 &     2.8 &     7.4 &   0.32 &   0.38 &       0.06 &  3.4584 &  3.4607 &    6.6660 &    6.5880 &       2 &             - &        6 &         1 \\
   9979905 & 0.338739 & 0.338739 &  457 &  220 &      2.5 &      2.3 &     7.9 &    11.3 &   0.46 &   0.69 &       0.23 &  2.9860 &  2.9788 &   29.5072 &   37.5023 &       2 &             - &        5 &         1 \\
   9987252 & 0.554550 & 0.554549 &  404 &  221 &      1.2 &      3.6 &     2.5 &    30.9 &   0.67 &   1.04 &       0.37 &  1.8399 &  1.8697 &   27.3224 &   15.0421 &       1 &             - &        6 &         1 \\
  10021274 & 0.576920 & 0.576932 &  214 &  839 &      2.6 &      3.6 &    11.5 &    43.7 &   0.75 &   1.12 &       0.37 &  1.7361 &  1.7396 &  357.1429 &  158.9825 &       1 &             - &        6 &         1 \\
  10030349 & 0.545073 & 0.545074 &  255 &  901 &      2.1 &      4.4 &     8.7 &    34.2 &   0.75 &   0.82 &       0.07 &  1.9187 &  1.9187 &   11.8984 &   11.8984 &       1 &             - &        5 &         1 \\
  10260828 & 0.380655 & 0.380643 &  280 &  862 &      2.2 &      7.4 &     5.3 &    77.3 &   0.35 &   0.49 &       0.14 &  2.6976 &  2.6306 &   14.1653 &  284.4950 &       2 &             - &        7 &         1 \\
  10399422 & 0.551844 & 0.551838 &  233 &  829 &      2.8 &      4.7 &    27.2 &    42.4 &   0.74 &   1.03 &       0.29 &  1.8797 &  1.8155 &   14.7885 &  299.4012 &       1 &             - &        6 &         1 \\
  10442149 & 0.519646 & 0.519648 &  209 &  377 &      1.2 &      2.5 &     2.2 &    11.9 &   0.96 &   0.77 &       0.19 &  1.9766 &  1.9635 &   19.1443 &   25.5591 &       1 &             - &        5 &         1 \\
  10481905 & 0.484720 & 0.484775 &  510 &  266 &      2.6 &      6.6 &    18.1 &    81.1 &   0.71 &   0.81 &       0.10 &  2.0970 &  2.1229 &   29.4898 &   16.6500 &       1 &             - &        8 &         1 \\
  10954700 & 0.594403 & 0.594391 &  422 &  194 &      1.5 &      6.1 &     4.8 &   138.3 &   0.70 &   0.96 &       0.26 &  1.6852 &  1.6879 &  355.8719 &  180.8318 &       1 &             - &        7 &         1 \\
  11151226 & 0.569182 & 0.569189 &  216 &  624 &      1.5 &      6.0 &     3.8 &    73.9 &   0.86 &   0.95 &       0.09 &  1.8082 &  1.8388 &   19.5027 &   12.2063 &       1 &             - &        6 &         1 \\
  11250867 & 0.649667 & 0.649714 &  182 & 1764 &      1.0 &      3.9 &     1.3 &    25.1 &   0.52 &   0.60 &       0.08 &  1.5731 &  1.5444 &   29.5727 &  188.6792 &       1 &             - &        7 &         1 \\
  11266421 & 0.621113 & 0.621119 &  241 &  512 &      1.7 &      4.0 &     6.8 &    36.8 &   0.80 &   0.62 &       0.18 &  1.6185 &  1.6237 &  117.9245 &   72.7802 &       1 &             - &        6 &         1 \\
  11281747 & 0.312089 & 0.312022 &  188 &  283 &      2.1 &      3.3 &     4.8 &    13.2 &   0.26 &   0.28 &       0.02 &  3.3036 &  3.3046 &   10.0664 &   10.0266 &       2 &             - &        6 &         1 \\
  11293454 & 0.568606 & 0.568598 &  307 &  511 &      2.2 &      5.2 &     8.2 &    51.6 &   0.62 &   0.83 &       0.21 &  1.7947 &  1.8401 &   27.7739 &   12.2933 &       1 &             - &        7 &         1 \\
  11644471 & 0.530138 & 0.530110 &  226 &  323 &      2.6 &      3.9 &    13.2 &    22.4 &   0.43 &   0.93 &       0.50 &  1.9446 &  1.9446 &   17.1615 &   17.1925 &       1 &             - &        8 &         1 \\
  11781491 & 0.541136 & 0.541136 &  210 &  478 &      1.7 &      6.7 &     9.1 &    93.8 &   0.64 &   0.84 &       0.20 &  1.8829 &  1.9253 &   28.5919 &   12.9308 &       1 &             - &        7 &         1 \\
  12172879 & 0.377286 & 0.377308 &  229 &  246 &      1.5 &      4.2 &     2.5 &    17.7 &   0.36 &   0.47 &       0.11 &  2.7239 &  2.6553 &   13.6305 &  202.8398 &       2 &             - &        7 &         1 \\
  12191421 & 0.577243 & 0.577226 &  228 &  506 &      2.3 &      5.5 &    17.4 &    64.0 &   0.69 &   0.93 &       0.24 &  1.8002 &  1.7359 &   14.7525 &  286.9440 &       1 &             - &        8 &         1 \\
  12246346 & 0.512537 & 0.512518 &  201 & 2117 &      1.3 &      3.1 &     2.4 &    32.8 &   0.87 &   0.87 &       0.00 &  1.9546 &  1.9769 &  282.8854 &   38.7747 &       1 &             - &        5 &         1 \\
  12359105 & 0.504674 & 0.504671 &  215 &  243 &      1.0 &      2.5 &     2.0 &     9.1 &   0.98 &   1.34 &       0.36 &  2.0240 &  2.0027 &   23.5073 &   47.2590 &       1 &             - &        5 &         1 \\
  12473468 & 0.561761 & 0.561765 &  177 & 1013 &      1.6 &      3.9 &     9.1 &    28.3 &   0.69 &   0.98 &       0.29 &  1.8519 &  1.7924 &   13.9383 &   81.3339 &       1 &             - &        6 &         1 \\
  12704270 & 0.478093 & 0.478109 &  250 &  223 &      1.3 &      3.1 &     3.2 &    11.7 &   0.78 &   0.81 &       0.03 &  2.1361 &  2.1360 &   22.5149 &   22.4871 &       1 &             - &        5 &         1 \\
  12968612 & 0.331995 & 0.331986 &  176 & 1120 &      1.3 &      2.4 &     2.3 &    13.7 &   0.37 &   0.54 &       0.17 &  3.0798 &  3.0169 &   14.7787 &  210.7482 &       2 &             - &        6 &         1 \\
  13227470 & 0.630186 & 0.630199 &  177 & 1752 &      1.4 &      2.5 &     2.8 &    10.9 &   0.62 &   0.83 &       0.21 &  1.6546 &  1.6429 &   14.7525 &   17.8285 &       1 &             - &        5 &         1 \\
  13331395 & 0.646706 & 0.646719 &  194 &  780 &      1.2 &      4.6 &     5.4 &    58.3 &   0.51 &   0.66 &       0.15 &  1.5518 &  1.5572 &  182.4818 &   91.4913 &       1 &             L &        0 &         2 \\
  13423223 & 0.634672 & 0.634669 &  254 &  872 &      0.8 &      2.3 &     0.9 &    17.9 &   0.71 &   1.04 &       0.33 &  1.6182 &  1.6242 &   23.4659 &   20.5698 &       1 &             - &        5 &         1 \\
  13517578 & 0.534375 & 0.534507 &  228 &  333 &      1.4 &      7.6 &     3.0 &   137.3 &   0.78 &   0.78 &       0.00 &  1.9036 &  1.9368 &   30.9598 &   15.1722 &       1 &             - &        7 &         1 \\
  13585738 & 0.475070 & 0.475040 &  224 &  993 &      5.9 &      5.6 &   121.4 &    42.9 &   0.83 &   0.61 &       0.22 &  2.1560 &  2.1563 &   19.5714 &   19.5408 &       1 &             - &        9 &         1 \\
  13587309 & 0.580910 & 0.580940 &  209 &  810 &      1.0 &      3.7 &     1.6 &    31.5 &   0.45 &   0.76 &       0.31 &  1.7892 &  1.7306 &   14.7591 &  108.1666 &       1 &             - &        8 &         1 \\
  13596315 & 0.490818 & 0.490832 &  158 & 1019 &      1.6 &      7.2 &     7.9 &   107.4 &   0.81 &   0.68 &       0.13 &  2.0719 &  2.0547 &   29.0023 &   57.7701 &       1 &             - &        7 &         1 \\
  13806757 & 0.652095 & 0.652121 &  225 &  605 &      1.4 &      3.4 &     4.5 &    33.4 &   0.78 &   0.76 &       0.02 &  1.5950 &  1.5948 &   16.2707 &   16.2906 &       1 &             - &        5 &         1 \\
  13811074 & 0.508439 & 0.508451 &  227 &  637 &      3.6 &      4.0 &    31.5 &    40.1 &   0.60 &   0.80 &       0.20 &  1.9848 &  1.9848 &   55.4939 &   55.5401 &       1 &             - &        7 &         1 \\
  13865387 & 0.381571 & 0.381609 &  215 &  788 &      0.7 &      3.5 &     0.5 &    15.7 &   0.38 &   0.51 &       0.13 &  2.6236 &  2.6620 &  350.8772 &   24.1022 &       2 &             - &        7 &         1 \\
  14155360 & 0.552032 & 0.552022 &  191 &  647 &      1.9 &      3.5 &     5.8 &    23.6 &   0.55 &   0.64 &       0.09 &  1.8143 &  1.8907 &  357.7818 &   12.6247 &       1 &             - &        5 &         1 \\
  14193913 & 0.565065 & 0.565083 &  224 &  510 &      5.2 &      9.5 &    54.9 &   128.1 &   0.78 &   1.02 &       0.24 &  1.8462 &  1.8046 &   13.0736 &   28.6123 &       1 &             - &        8 &         1 \\
  14211532 & 0.496891 & 0.496879 &  186 &  541 &      1.1 &      7.1 &     2.2 &   117.8 &   0.62 &   1.02 &       0.40 &  2.0463 &  2.0162 &   29.6340 &  275.8621 &       1 &             - &        7 &         1 \\
  14225011 & 0.610380 & 0.610382 &  167 & 1819 &      1.0 &      1.1 &     1.2 &     2.4 &   0.69 &   0.92 &       0.23 &  1.6486 &  1.6436 &   96.9462 &  187.9699 &       1 &             L &        0 &         2 \\
  14299756 & 0.530149 & 0.530152 &  225 & 2072 &      1.2 &      3.7 &     1.9 &    43.7 &   0.93 &   1.15 &       0.22 &  1.9201 &  1.9445 &   29.5552 &   17.1777 &       1 &             - &        6 &         1 \\
  14303456 & 0.546045 & 0.546015 &  212 &  995 &      1.2 &      2.5 &     2.5 &    14.2 &   0.76 &   0.70 &       0.06 &  1.9170 &  1.9171 &   11.6761 &   11.6809 &       1 &             - &        6 &         1 \\
  14310401 & 0.594513 & 0.594591 &  220 & 1028 &      1.6 &      4.5 &     4.8 &    51.0 &   0.86 &   0.54 &       0.32 &  1.7173 &  1.6852 &   28.3970 &  293.2551 &       1 &             - &        8 &         1 \\
  14396814 & 0.483136 & 0.483141 &  205 & 1042 &      1.5 &      4.9 &     3.5 &    75.6 &   0.78 &   1.06 &       0.28 &  2.1037 &  2.1033 &   29.4724 &   29.8151 &       1 &             - &        6 &         1 \\
  14520582 & 0.644803 & 0.644773 &  184 &  638 &      1.8 &      4.0 &    11.9 &    50.9 &   0.74 &   0.62 &       0.12 &  1.5878 &  1.5830 &   27.0709 &   31.1915 &       1 &             - &        7 &         1 \\
  14758749 & 0.536492 & 0.536476 &  175 & 1097 &      1.1 &      4.4 &     1.5 &    56.9 &   0.91 &   1.07 &       0.16 &  1.9333 &  1.9334 &   14.4279 &   14.4207 &       1 &             - &        7 &         1 \\
  15009461 & 0.599300 & 0.599317 &  216 &  523 &      2.7 &      2.9 &    27.4 &    14.0 &   0.58 &   0.48 &       0.10 &  1.7083 &  1.6822 &   25.1953 &   73.4484 &       1 &             - &        5 &         1 \\
  15099715 & 0.528171 & 0.528154 &  203 &  969 &      1.3 &      4.9 &     2.2 &    40.8 &   0.80 &   1.01 &       0.21 &  1.9480 &  1.9480 &   18.2932 &   18.2999 &       1 &             - &        7 &         1 \\
  15134836 & 0.570079 & 0.570085 &  197 &  997 &      1.0 &      3.2 &     3.0 &    29.0 &   0.80 &   0.86 &       0.06 &  1.8262 &  1.8370 &   13.8812 &   12.0707 &       1 &             - &        5 &         1 \\
  15661449 & 0.364648 & 0.364726 &  156 &  595 &      3.4 &      5.7 &    11.0 &    34.9 &   0.37 &   0.30 &       0.07 &  2.8168 &  2.7456 &   13.4418 &  264.9007 &       2 &             - &        8 &         1 \\
  15958022 & 0.573521 & 0.573540 &  160 & 1084 &      0.9 &      3.1 &     0.9 &    24.1 &   0.65 &   0.90 &       0.25 &  1.8038 &  1.7469 &   16.6030 &  297.1768 &       1 &             - &        7 &         1 \\
  16021203 & 0.357159 & 0.357209 &  188 &  340 &      0.8 &      2.5 &     1.0 &     9.3 &   0.38 &   0.53 &       0.15 &  2.9027 &  2.9024 &    9.7272 &    9.7158 &       2 &             - &        5 &         1 \\
  16039295 & 0.327033 & 0.327042 &  173 &  241 &      1.1 &      2.1 &     1.7 &     7.2 &   0.35 &   0.51 &       0.16 &  3.0826 &  3.0839 &   40.2414 &   38.1679 &       2 &             - &        6 &         1 \\
  16208287 & 0.294033 & 0.294020 &  150 &  365 &      2.2 &      3.6 &     8.0 &    25.8 &   0.38 &   0.56 &       0.18 &  3.4716 &  3.4116 &   14.1653 &   95.5110 &       2 &             - &        7 &         1 \\
  16259674 & 0.575146 & 0.575151 &  179 &  362 &      0.8 &      1.7 &     1.3 &     3.4 &   0.73 &   0.56 &       0.17 &  1.7654 &  1.7429 &   37.4322 &  234.7418 &       1 &             L &        0 &         2 \\
  16300450 & 0.335615 & 0.335595 &  203 & 1315 &      2.1 &      5.8 &    12.9 &    45.1 &   0.47 &   0.66 &       0.19 &  2.9824 &  2.9927 &  355.8719 &   77.6699 &       2 &             - &        9 &         1 \\
  16554726 & 0.310226 & 0.310235 &  231 &  549 &      1.3 &      8.0 &     2.3 &    75.7 &   0.38 &   0.44 &       0.06 &  3.2916 &  3.2275 &   14.6714 &  240.6739 &       2 &             - &        7 &         1 \\
  16600479 & 0.555616 & 0.555608 &  182 &  732 &      1.3 &      3.2 &     3.1 &    29.6 &   0.85 &   0.63 &       0.22 &  1.8555 &  1.8033 &   17.9598 &  286.5330 &       1 &             - &        6 &         1 \\
  16659561 & 0.420350 & 0.420374 &  201 & 2495 &      0.7 &      2.4 &     0.5 &     7.6 &   0.39 &   0.51 &       0.12 &  2.4859 &  2.3892 &    9.3484 &   96.6184 &       2 &             - &        6 &         1 \\
  17009525 & 0.569504 & 0.569510 &  517 &  237 &      0.9 &      2.6 &     1.1 &    15.2 &   0.56 &   0.82 &       0.26 &  1.7898 &  1.7649 &   29.4811 &  111.3586 &       1 &             - &        5 &         1 \\
  17082877 & 0.358479 & 0.358483 &  485 &  432 &      1.0 &      2.4 &     1.2 &    10.4 &   0.30 &   0.49 &       0.19 &  2.8235 &  2.7924 &   29.4724 &  350.2627 &       2 &             - &        5 &         1 \\
  17185566 & 0.614160 & 0.614169 &  542 &  629 &      1.5 &      1.9 &     3.2 &     6.2 &   0.40 &   0.42 &       0.02 &  1.6620 &  1.6365 &   29.5814 &  120.6273 &       1 &             Z &        0 &         2 \\
  17275627 & 0.537775 & 0.537771 &  563 &  474 &      2.1 &      4.8 &     7.8 &    27.7 &   0.74 &   1.00 &       0.26 &  1.8934 &  1.9311 &   29.5029 &   13.9665 &       1 &             - &        6 &         1 \\
  17302403 & 0.488261 & 0.488343 &  328 &  629 &      2.0 &      6.4 &    11.0 &    74.4 &   0.73 &   0.63 &       0.10 &  2.1187 &  2.0703 &   14.1653 &   44.3754 &       1 &             - &        8 &         1 \\
  17544856 & 0.614297 & 0.614296 &  533 &  537 &      2.0 &      3.4 &     9.6 &    20.9 &   0.59 &   0.77 &       0.18 &  1.6618 &  1.6327 &   29.5072 &  206.3983 &       1 &             - &        6 &         1 \\
  17880250 & 0.466539 & 0.466506 &  234 & 1066 &      1.6 &      3.7 &     6.3 &    27.5 &   1.05 &   0.86 &       0.19 &  2.1463 &  2.2140 &  352.7337 &   14.1955 &       1 &             - &        8 &         1 \\
  17919686 & 0.508665 & 0.508712 &  204 & 1739 &      4.2 &      4.9 &    41.5 &    57.2 &   0.71 &   0.75 &       0.04 &  1.9843 &  1.9842 &   54.4070 &   54.0833 &       1 &             - &        7 &         1 \\
  17981455 & 0.369450 & 0.369531 &  156 & 1069 &      2.1 &      8.3 &     7.3 &    78.1 &   0.37 &   0.41 &       0.04 &  2.8136 &  2.7095 &    9.3523 &  299.8501 &       2 &             - &        7 &         1 \\
  18102636 & 0.351465 & 0.351482 &  213 & 1313 &      1.0 &      3.3 &     1.0 &    16.4 &   0.50 &   0.60 &       0.10 &  2.9468 &  2.9239 &    9.8445 &   12.6839 &       2 &             - &        7 &         1 \\
  18465689 & 0.547884 & 0.547895 &  215 & 1391 &      1.2 &      3.7 &     2.6 &    26.1 &   0.54 &   0.62 &       0.08 &  1.8594 &  1.8306 &   29.2869 &  184.5018 &       1 &             - &        5 &         1 \\
  18616226 & 0.382200 & 0.382179 &  188 &  724 &      1.3 &      2.1 &     1.5 &     5.9 &   0.41 &   0.36 &       0.05 &  2.6819 &  2.6916 &   15.2648 &   13.3316 &       2 &             - &        5 &         1 \\
  18682363 & 0.550246 & 0.550252 &  226 &  977 &      0.8 &      1.9 &     1.0 &     6.1 &   0.92 &   1.15 &       0.23 &  1.8277 &  1.8791 &   96.8992 &   16.1865 &       1 &             L &        0 &         2 \\
  18836175 & 0.544014 & 0.544001 &  212 & 2727 &      1.8 &      4.6 &     4.5 &    41.0 &   0.73 &   0.66 &       0.07 &  1.9033 &  1.9205 &   15.3516 &   12.1595 &       1 &             - &        5 &         1 \\
  18870159 & 0.531439 & 0.531407 &  205 & 2861 &      1.0 &      4.2 &     1.3 &    23.8 &   0.71 &   0.93 &       0.22 &  1.9492 &  1.9422 &   14.8006 &   16.5426 &       1 &             - &        8 &         1 \\
  18870268 & 0.589831 & 0.589804 &  202 & 2797 &      0.9 &      3.2 &     1.1 &    15.5 &   0.76 &   0.85 &       0.09 &  1.7294 &  1.7373 &   29.4247 &   23.8977 &       1 &             - &        7 &         1 \\
  18875199 & 0.634381 & 0.634380 &  228 & 2781 &      0.8 &      2.9 &     1.3 &    13.4 &   0.81 &   1.06 &       0.25 &  1.6254 &  1.6263 &   20.3915 &   20.0040 &       1 &             - &        5 &         1 \\
  19356745 & 0.549451 & 0.549431 &  233 &  746 &      1.4 &      2.6 &     3.1 &    18.8 &   0.84 &   0.74 &       0.10 &  1.8228 &  1.8809 &  355.8719 &   16.4285 &       1 &             - &        5 &         1 \\
  19372092 & 0.601367 & 0.601375 &  193 & 1178 &      0.8 &      3.3 &     1.1 &    26.7 &   0.59 &   0.47 &       0.12 &  1.6933 &  1.6664 &   32.8407 &  283.2861 &       1 &             - &        5 &         1 \\
  19403325 & 0.656846 & 0.656853 &  236 & 2132 &      1.0 &      2.1 &     1.0 &    11.3 &   0.68 &   0.96 &       0.28 &  1.5694 &  1.5619 &   21.3015 &   25.3485 &       1 &             - &        5 &         1 \\
  19408994 & 0.649740 & 0.649804 &  217 & 1219 &      1.3 &      5.1 &     3.0 &    80.0 &   0.79 &   0.63 &       0.16 &  1.6018 &  1.6113 &   15.9426 &   13.8102 &       1 &             - &        9 &         1 \\
  19466437 & 0.542637 & 0.542515 &  208 & 1270 &      1.0 &      2.8 &     2.2 &    31.7 &   1.14 &   1.49 &       0.35 &  1.9228 &  1.9230 &   12.5117 &   12.5423 &       1 &             - &        7 &         1 \\
  19773423 & 0.476257 & 0.476279 &  240 &  920 &      1.5 &      5.4 &     5.5 &    91.1 &   0.86 &   1.18 &       0.32 &  2.1482 &  2.1481 &   20.6228 &   20.6356 &       1 &             - &        9 &         1 \\
  19775800 & 0.310856 & 0.310867 &  292 & 2583 &      1.3 &      2.7 &     2.2 &    15.1 &   0.46 &   0.60 &       0.14 &  3.2846 &  3.3225 &   14.7700 &    9.4630 &       2 &             - &        5 &         1 \\
  19780691 & 0.637441 & 0.637437 &  238 & 2606 &      1.0 &      3.1 &     2.4 &    32.7 &   0.75 &   1.17 &       0.42 &  1.5812 &  1.6128 &   80.1925 &   22.6963 &       1 &             - &        6 &         1 \\
  19806944 & 0.513789 & 0.513787 &  198 & 3881 &      1.5 &      2.6 &     4.0 &    18.3 &   0.83 &   0.94 &       0.11 &  1.9746 &  2.0028 &   35.4233 &   17.7195 &       1 &             L &        0 &         2 \\
  19902731 & 0.306250 & 0.306302 &  164 & 1469 &      1.0 &      2.6 &     1.0 &    12.1 &   0.43 &   0.57 &       0.14 &  3.4029 &  3.3944 &    7.2664 &    7.7125 &       2 &             - &        6 &         1 \\
  19925031 & 0.361735 & 0.361726 &  189 &  627 &      0.9 &      3.4 &     1.2 &    13.5 &   0.46 &   0.53 &       0.07 &  2.8040 &  2.7983 &   25.2781 &   29.5858 &       2 &             - &        5 &         1 \\
  20107944 & 0.598481 & 0.598468 &  215 & 1343 &      1.1 &      3.1 &     1.3 &    30.0 &   0.61 &   0.77 &       0.16 &  1.6744 &  1.6789 &  287.7698 &  126.2626 &       1 &             L &        0 &         2 \\
  20271572 & 0.536805 & 0.536792 &  181 & 2302 &      1.4 &      6.3 &     3.1 &    95.5 &   0.67 &   0.83 &       0.16 &  1.9328 &  1.9328 &   14.3102 &   14.3062 &       1 &             - &        7 &         1 \\
  20441941 & 0.688814 & 0.688836 &  187 & 1573 &      3.5 &      5.6 &    10.8 &    57.3 &   0.48 &   0.45 &       0.03 &  1.5194 &  1.4858 &   14.7809 &   29.3858 &       1 &             - &        6 &         1 \\
  20815762 & 0.728292 & 0.728292 &  188 & 1109 &      1.1 &      2.1 &     1.3 &     5.4 &   0.50 &   0.69 &       0.19 &  1.4070 &  1.3786 &   29.5029 &  181.3237 &       1 &             - &        5 &         1 \\
  21010711 & 0.488102 & 0.488058 &  198 & 1207 &      1.2 &      8.0 &     4.6 &   186.9 &   1.09 &   1.15 &       0.06 &  2.0717 &  2.0720 &   43.5635 &   43.2807 &       1 &             L &        0 &         2 \\
  21011352 & 0.326046 & 0.326018 &  187 & 2690 &      1.9 &      2.5 &     6.0 &    11.2 &   0.44 &   0.43 &       0.01 &  3.0992 &  3.0983 &   31.0607 &   32.3258 &       2 &             - &        5 &         1 \\
  21080566 & 0.556566 & 0.556565 &  239 &  587 &      0.9 &      2.6 &     1.1 &    19.7 &   0.88 &   1.05 &       0.17 &  1.8660 &  1.8076 &   14.4394 &   92.1659 &       1 &             - &        5 &         1 \\
  21215819 & 0.524380 & 0.524392 &  575 &  272 &      1.1 &      4.0 &     2.4 &    33.4 &   0.83 &   1.01 &       0.18 &  1.9549 &  1.9549 &   20.8986 &   20.8638 &       1 &             - &        6 &         1 \\
  21488669 & 0.501644 & 0.501661 &  473 &  449 &      1.9 &      5.7 &    10.9 &    52.6 &   0.68 &   0.61 &       0.07 &  2.0026 &  1.9981 &  108.9918 &  211.1932 &       1 &             - &        7 &         1 \\
  21556651 & 0.614826 & 0.614808 &  572 &  450 &      1.8 &      3.1 &     6.5 &    19.1 &   0.66 &   0.57 &       0.09 &  1.6630 &  1.6295 &   27.3523 &  335.5705 &       1 &             - &        6 &         1 \\
  21619184 & 0.557343 & 0.557320 &  335 &  605 &      2.3 &      3.7 &    10.1 &    21.3 &   0.68 &   0.64 &       0.04 &  1.8309 &  1.7972 &   27.2926 &  341.2969 &       1 &             - &        5 &         1 \\
  21640723 & 0.650454 & 0.650489 &  460 &  431 &      1.0 &      2.8 &     2.0 &    15.6 &   0.60 &   0.60 &       0.00 &  1.6067 &  1.6065 &   14.4248 &   14.4561 &       1 &             - &        5 &         1 \\
  21688272 & 0.304803 & 0.304790 &  263 &  498 &      2.3 &      1.8 &    10.4 &     5.9 &   0.43 &   0.56 &       0.13 &  3.3515 &  3.2859 &   14.1493 &  203.4588 &       2 &             - &        5 &         1 \\
  21806402 & 0.592081 & 0.592104 &  592 &  260 &      1.6 &      6.2 &     7.4 &    90.8 &   0.55 &   0.69 &       0.14 &  1.7228 &  1.7033 &   29.5902 &   69.5410 &       1 &             - &        7 &         1 \\
  21869616 & 0.518196 & 0.518199 &  599 &  420 &      1.4 &      3.7 &     5.0 &    33.2 &   0.93 &   0.79 &       0.14 &  1.9663 &  1.9662 &   27.3860 &   27.4123 &       1 &             - &        5 &         1 \\
  21874209 & 0.611295 & 0.611286 &  593 &  201 &      2.5 &      5.9 &    17.9 &    67.6 &   0.59 &   0.88 &       0.29 &  1.6698 &  1.6887 &   29.4985 &   18.9520 &       1 &             - &        7 &         1 \\
  21947560 & 0.480496 & 0.480497 &  322 &  540 &      2.5 &      4.2 &    12.7 &    34.4 &   0.76 &   0.88 &       0.12 &  2.1190 &  2.1204 &   26.4306 &   25.4972 &       1 &             - &        5 &         1 \\
  21967825 & 0.540607 & 0.540600 &  263 &  363 &      1.8 &      4.7 &     6.7 &    60.2 &   0.63 &   0.97 &       0.34 &  1.9263 &  1.9263 &   13.0736 &   13.0745 &       1 &             - &        6 &         1 \\
  22244513 & 0.604149 & 0.604077 &  330 &  265 &      2.5 &      8.1 &     9.2 &   130.0 &   0.45 &   0.78 &       0.33 &  1.6951 &  1.6736 &   25.0627 &   54.8697 &       1 &             - &        9 &         1 \\
  22542105 & 0.574095 & 0.574110 &  537 &  402 &      3.2 &      2.2 &    19.7 &    13.6 &   0.56 &   0.56 &       0.00 &  1.7757 &  1.7473 &   29.5334 &  181.1594 &       1 &             - &        5 &         1 \\
  22714229 & 0.327808 & 0.327810 &  282 &  518 &      3.3 &      1.2 &    16.1 &     1.5 &   0.33 &   0.50 &       0.17 &  3.1211 &  3.0730 &   14.1733 &   44.5236 &       2 &             - &        6 &         1 \\
  22944851 & 0.582094 & 0.582078 &  323 &  349 &      1.0 &      2.6 &     2.2 &    15.1 &   0.56 &   0.83 &       0.27 &  1.7545 &  1.7209 &   27.3785 &  341.2969 &       1 &             - &        6 &         1 \\
  22959674 & 0.405333 & 0.405409 &  274 &  556 &      1.8 &      3.8 &     3.8 &    21.6 &   0.30 &   0.31 &       0.01 &  2.5377 &  2.4802 &   14.1733 &   73.9919 &       2 &             - &        6 &         1 \\
  23166739 & 0.543359 & 0.543368 &  444 &  404 &      1.5 &      2.3 &     6.5 &     9.7 &   0.83 &   0.54 &       0.29 &  1.8743 &  1.8459 &   29.5072 &  181.4882 &       1 &             - &        5 &         1 \\
  23184808 & 0.338821 & 0.338888 &  540 &  253 &      1.0 &      5.7 &     1.9 &    40.8 &   0.42 &   0.48 &       0.06 &  2.9852 &  2.9782 &   29.5639 &   36.5297 &       2 &             - &        8 &         1 \\
  23193507 & 0.473158 & 0.473174 &  559 &  208 &      3.4 &      4.6 &    54.2 &    42.8 &   0.78 &   1.13 &       0.35 &  2.1688 &  2.1687 &   18.0717 &   18.0783 &       1 &             - &        8 &         1 \\
  23252474 & 0.451658 & 0.451674 &  287 &  434 &      1.2 &      4.9 &     3.6 &    50.4 &   0.88 &   0.72 &       0.16 &  2.2506 &  2.2223 &   27.3486 &  120.4094 &       1 &             - &        7 &         1 \\
  23435891 & 0.482831 & 0.482808 &  233 & 1160 &      4.0 &      7.4 &    46.6 &    94.2 &   0.82 &   0.97 &       0.15 &  2.1404 &  2.1055 &   14.4259 &   29.1843 &       1 &             - &        7 &         1 \\
  23624228 & 0.364453 & 0.364454 &  295 &  471 &      3.8 &      5.3 &    23.2 &    30.6 &   0.32 &   0.35 &       0.03 &  2.8143 &  2.7655 &   14.1854 &   46.1574 &       2 &             - &        5 &         1 \\
  23653629 & 0.442052 & 0.442055 &  299 &  516 &      2.4 &      4.4 &    15.8 &    47.4 &   0.82 &   0.74 &       0.08 &  2.3330 &  2.2839 &   14.1233 &   46.0405 &       1 &             - &        5 &         1 \\
  23846316 & 0.588263 & 0.588260 &  388 &  202 &      1.2 &      2.8 &     3.0 &    30.5 &   0.74 &   1.12 &       0.38 &  1.7339 &  1.7484 &   29.4204 &   20.6271 &       1 &             - &        5 &         1 \\
  23898397 & 0.563018 & 0.562989 &  323 &  439 &      1.6 &      3.5 &     7.0 &    38.5 &   0.69 &   0.60 &       0.09 &  1.7793 &  1.8094 &  318.4713 &   30.1477 &       1 &             - &        7 &         1 \\
  24020106 & 0.542397 & 0.542396 &  584 &  209 &      2.9 &      4.5 &    16.0 &    54.3 &   0.52 &   0.95 &       0.43 &  1.8776 &  1.9232 &   29.4855 &   12.5778 &       1 &             - &        6 &         1 \\
  24216004 & 0.382077 & 0.381912 &  546 &  287 &      1.9 &      7.8 &     6.5 &   110.6 &   0.30 &   0.44 &       0.14 &  2.6511 &  2.6244 &   29.5596 &  167.2241 &       2 &             - &        8 &         1 \\
\bottomrule
\end{tabular}
\end{center}

